Devign: Effective Vulnerability Identification by Learning Comprehensive Program Semantics via Graph Neural Networks

Vulnerability identification is crucial to protect the software systems from attacks for cyber security. It is especially important to localize the vulnerable functions among the source code to facilitate the fix. However, it is a challenging and tedious process, and also requires specialized security expertise. Inspired by the work on manually-defined patterns of vulnerabilities from various code representation graphs and the recent advance on graph neural networks, we propose Devign, a general graph neural network based model for graph-level classification through learning on a rich set of code semantic representations. It includes a novel Conv module to efficiently extract useful features in the learned rich node representations for graph-level classification. The model is trained over manually labeled datasets built on 4 diversified large-scale open-source C projects that incorporate high complexity and variety of real source code instead of synthesis code used in previous works. The results of the extensive evaluation on the datasets demonstrate that Devign outperforms the state of the arts significantly with an average of 10.51% higher accuracy and 8.68\% F1 score, increases averagely 4.66% accuracy and 6.37% F1 by the Conv module.

==> approach.tex <==



In literature, most machine learning or pattern based approaches \cite{nguyen10,yamaguchi2014,ndss18vuldeepecker,dam2017automatic} predict vulnerability at the coarse granularity level of a source file or an application, i.e., whether a source file or an application is potentially vulnerable or not. In our task, we chose to analyze vulnerable code at the \textit{function level} which is the finest level of granularity in the overall flow of vulnerability analysis.
%Inspired by previous works that define handcraft vulnerability patterns from dependency and code property graphs to match similar patterns in source code, our work aims to represent the source code in graphs and automatically learn all the possible vulnerable patterns using graph neural networks.
%\ning{check if i alternate the original meaning:}
Vulnerability patterns manually crafted with the code property graphs, integrating all syntax and dependency semantics, have been proved to be one of the most effective approaches \cite{yamaguchi2014}.
Inspired by this, we aim to represent the source code in graphs and automate the learning and detection of all the possible vulnerable patterns using graph neural networks.
%In this section, we describe the detailed approach of the graph neural network-based vulnerability detection problem.
Our graph neural network based approach to detect vulnerable functions includes the following components, which are explained in the remainder of this section.
\begin{itemize}
    \setlength\itemsep{0.01em}
    \item \textbf{Code Representation}, which encodes the raw source code of a function into a joint graph structure with comprehensive program semantics. %(See Section~\ref{sec:code})
    \item \textbf{Learning Node Representation}, which learns the features of nodes in a graph through graph neural networks.
   %  (See Section~\ref{sec:node})
    \item \textbf{Graph-level Classification}, which leverages all individual node representations of a graph to determine if a function represented by the graph is vulnerable or not.
\end{itemize}



\subsection{Code Representation}
\label{sec:code}
In program analysis, various representations of the program are utilized to manifest deeper information behind the textual code, where classic concepts include ASTs, control flow graphs, and data flow graphs that capture the syntactic and semantic relationships among the different elements of the source code. 
Many vulnerabilities such as memory disclosure are too implicit to be spotted without a joint consideration of the structure, control flow and data dependencies of code \cite{yamaguchi2014}.  
%As shown in \cite{yamaguchi2014}, a combination of these code-representation graphs, named \textit{code property graph}, enables to model a broader range of vulnerability types. 
For example, it is reported that ASTs alone can be used to find only insecure arguments.  While combining ASTs with control flow graphs, it enables to cover two more types of vulnerabilities, i.e., resource leaks and some use-after-free vulnerabilities. By further integrating the ASTs, control flow graphs and data flow graphs, it is possible to describe most types of vulnerabilities except two that require information other than static code (race condition depends on runtime properties and design errors are hard to model without details on the intended design of a program). 

Though \cite{yamaguchi2014} \emph{manually} crafted the vulnerability templates  in the form of graph traversals, it conveyed the key insight and proved the feasibility to learn a broader range of vulnerability patterns through integrating properties of ASTs, control flow graphs and data flow graphs into a joint data structure. Based on this insight, this work attempts to automatically mine extensive vulnerability patterns from comprehensive code representations. 
Beside the three classical code structures, we also take the natural sequence of source code into consideration, since the recent advance on deep learning based vulnerability detection has demonstrated its usability ~\cite{ndss18vuldeepecker,russell2018automated}. 
It can complement the classical  representations because its unique flat structure captures the relationships of code tokens in `human-readable' source code.
%The natural sequence reflects the direct order of  AST leaf nodes and  

Next we briefly introduce each type of the code representations and how we embed various types of graphs into one joint graph, following a code example of integer overflow as in Figure~\ref{fig:graph_representation}(a) and its graph representation as shown in Figure~\ref{fig:graph_representation}(b).
%as shown in Fig.~\ref{fig:graph_representation} via an example of integer overflow in Listing~\ref{snippet}.



% \begin{lstlisting}[float,language=C,caption={A code example of integer overflow},basicstyle=\footnotesize,label=snippet]
% short add (short b){
%   short a = 32768;
%   short c = a + b;
%   return c;
% }
% \end{lstlisting}

\begin{comment}
\begin{lstlisting}[float,language=C,caption={A code example of integer overflow},basicstyle=\fontsize{13}{13}\selectfont\ttfamily,label=snippet]
short add (short b) {
   short a = 32767;
   if (b > 0){
        a = a + b;
   }
   return a;
}
\end{lstlisting}
\end{comment}
%\begin{comment}

%\end{comment}

\begin{comment}

\begin{figure*}[t!]
    \begin{minipage}[b]{0.2\textwidth}
    \centering
        \includegraphics[scale=0.35]{graph_listing.eps}
        \caption{Code snippet of integer overflow}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.8\textwidth}
    \centering
        \includegraphics[scale=0.25]{graph_representation.eps}
        \caption{Graph Representation of Code Snippet in Listing 1}
    \end{minipage}
  %  \caption{Caption place holder}
\end{figure*}
\end{comment}



\begin{figure*}[htb]
     \centering
     \includegraphics[width=1\textwidth]{figures/overflow_graph_new.eps}
     \caption{Graph Representation of Code Snippet with Integer Overflow } 
     \label{fig:graph_representation}
     \vspace{-0.1in}
\end{figure*}
\begin{description}
\setlength\itemsep{0.01in}
    \item[Abstract Syntax Tree (AST)] AST is an ordered tree representation structure of source code. Usually, it is the first-step representation used by code parsers to understand the fundamental structure of the program and to examine syntactic errors. Hence, it forms the basis for the generation of many other code representations. 
    Starting from the root node, the codes are broken down into code blocks, statements, declaration, expressions and etc., and finally into the primary tokens.
    These tokens form the leaf nodes in ASTs.
    We call edges representing the directed child-parent relationship in AST \textit{Child} edge.
    The major AST nodes are shown in Figure~\ref{fig:graph_representation}.
    All the boxes are AST nodes, with specific codes in the first line and node type annotated. The blue boxes are leaf nodes of AST and purple arrows represent the child-parent relations.
    \item[Control Flow Graph (CFG)] CFG describes the possible orders in which code statements can be executed. 
    The path alternatives are determined by conditional statements, e.g., \textit{if}, \textit{for}, and \textit{switch} statements. In CFGs, nodes denote statements and conditions, and they are connected by directed \textit{Control} edges to indicate the transfer of control. The control edges are highlighted with green arrows in Figure~\ref{fig:graph_representation}. Particularly, the flow starts from the entry and ends at the exit, and two different paths derive at the \textit{if} statements.
    %CFG is the graph that can represent the flow of the program based on the source code. It records the possible paths that the program might traverse. 
    %Generally, these two graph structures could represent source codes efficiently. 
    \item[Data Flow Graph (DFG)] DFG tracks the usage of variables throughout the CFG. Data flow is variable oriented and any data flow involves the reading or writing of certain variables. A DFG edge represents the subsequent reading or writing onto the same variables. It is illustrated by orange double arrows in Figure~\ref{fig:graph_representation} and with the involved variables annotated over the edge. For example, the parameter $b$ is used in both the \textit{if} condition and the assignment statement.
    %However, such representation is too coarse to be used in machine learning since the 
    \item[Natural Code Sequence] In order to encode the natural sequential order of the source code, we use \textit{NextToken} edges to connect neighboring code tokens in the ASTs. There are two benefits with such encoding, one is to reserve the programming logic reflected by the sequence of source code, the other is to keep it as precise as possible to only the key tokens. The \textit{NextToken} edges are denoted by red arrows in Figure~\ref{fig:graph_representation}, string up all the leaf nodes of the AST.%In Figure~\ref{fig:graph_representation}, the NextToken edges are represented by pink dotted line and the nodes are colored with pink. 
\end{description}




\begin{figure*}[htb]
     \centering
     \includegraphics[width=0.8\textwidth]{figures/network.eps}
     \caption{The Architecture of Devign  with CNN Classifiers}
     \label{fig:network}
     \vspace{-0.1in}
\end{figure*}

\vspace{-0.02in}
\subsection{Gated Graph Neural Network Model}\label{sec:node}
Our network model builds upon the Gated Graph Neural Networks (GGNN) which extends Graph Neural Networks to output sequences \cite{li2015gated}. We modify and improve it for the problem of graph classification.  We first formulate the problem, and then introduce the network model.

\noindent \textbf{Problem Formulation} We denote a function $F$ in source code as a multi-edged graph $G=(V,E)$, where each vertex $v$ in $V$ denotes a node in the graph, and each edge $e_{i,j}^{t} \in E_t$ denotes that node $v_i, v_j$ is connected via an edge of type $t$ where $t$ is an integer and $0 \leq t\leq T$. The total number of edge types $T$ denotes all the number of the integrated graph representations to facilitate vulnerability discovery. Therefore, given $G=(V,E)$ for $F$, we aim to predict whether $F$ is vulnerable or not.

\noindent \textbf{Learning Node Representations} We summarize the basics of GGNN here. Given a graph $G = (V, E)$, let ${x_i \in X}$ be the real-valued vectors of node features where each node $i$ associates with an annotation $x_i$ representing the initial feature of the node. For each node $i\in V$, we then initialize the node state vector $h_i$ using the initial annotation by copying $x_i$ into the first dimensions and padding extra 0's to allow hidden states that are larger than the annotation size, i.e., $h_i = [x_i^\top, \mathbf{0}]^\top$. To propagate information throughout graphs, at each time step $t$, all nodes communicate with each other by passing information via edges dependent on the edge type and direction (described by the adjacent matrix $A$), i.e.,
\begin{equation}
    a_i^t = A_i^\top \bigg[h_1^{(t-1)\top},\dots,h_{|V|}^{(t-1)\top}\bigg] + b
\end{equation}
where $b$ is the biases. In particular, a new state for a node $i$ is calculated by aggregating all types of incoming information. The remaining steps are gated recurrent unit (GRU) like updates that incorporate information from the other nodes and the previous time step to update a node's hidden state $h_i^t$. The above propagation procedure iterates over a fixed number of time steps, and the state vectors at the last time step is the final node representation.

\noindent \textbf{Graph-level Classification} The generated node embeddings by GGNNs can be used as input to any prediction layer, e.g., for node classification or link prediction or graph-level classification, and then the whole model can be trained in an end-to-end fashion. In our approach, we require to perform the task of graph-level classification to determine whether an input function is vulnerable or not. 
The standard approach to graph classification is gathering all these generated node embeddings globally, e.g., using a linear weighted summation to flatly adding up all the embeddings  \cite{li2015gated,dai2016discriminative}. Consequently, this approach hinders effective classification over entire graphs \cite{ying2018hierarchical,zhang2018end}. Since our node representations are both semantic and structural, learned from GRU-like graph neural networks instead of graph convolution networks that need a sortpooling layer to sort the structural node features in a consistent vertex ordering before inputting into traditional CNNs, we directly apply 1-D convolution layers and dense layers for more effective prediction\footnote{We also tried  LSTMs and BiLSTMs (with and without attention mechanisms) on the ordered nodes to classify, however, the CNN classifiers work best overall.}. Figure~\ref{fig:network} illustrates the modified network architecture.  %The network structure is shown in Fig. \ref{fig:network}  

